Data Distribution Bottlenecks in Grounding Language Models to Knowledge Bases

Language models (LMs) have already demonstrated remarkable abilities in understanding and generating both natural and formal language. Despite these advances, their integration with real-world environments such as large-scale knowledge bases (KBs) remains an underdeveloped area, affecting applications such as semantic parsing and indulging in "hallucinated" information. This paper is an experimental investigation aimed at uncovering the robustness challenges that LMs encounter when tasked with knowledge base question answering (KBQA). The investigation covers scenarios with inconsistent data distribution between training and inference, such as generalization to unseen domains, adaptation to various language variations, and transferability across different datasets. Our comprehensive experiments reveal that even when employed with our proposed data augmentation techniques, advanced small and large language models exhibit poor performance in various dimensions. While the LM is a promising technology, the robustness of the current form in dealing with complex environments is fragile and of limited practicality because of the data distribution issue. This calls for future research on data collection and LM learning paradims.

==> backup/introduction0108.tex <==
Knowledge base question answering (KBQA) aims to answer natural language questions based on knowledge bases (KBs) such as DBpedia \cite{Lehmann15dbpedia}, Freebase \cite{bollacker08freebase} and Wikidata \cite{vrandecic14wikidata}. 
It allows users to query the KB through natural language without having to learn a complex formal query language.
Extensive research has been conducted on KBQA leaderboards and models \cite{lan21complex}, with datasets ranging from small, single-hop to large, multi-hop with numerical calculations.
While KBQA models continue to evolve to address the increasing complexity of the dataset, the form of data collection and evaluation protocols has rarely changed.
More importantly, the lack of reflection on the whole leaderboard building process makes some critical realities overlooked.

KBQA leaderboards usually involve only limited query patterns and abbreviated evaluation metrics, but the QA demands in reality are diverse and difficult to summarize.
In this work, we argue that KBQA leaderboards do not yet simulate real-world scenarios well. % metrics do not always reflect model performance in real-world scenarios.
Thus, we systematically investigate KBQA leaderboards in terms of the practicality of the \textbf{dataset construction} and \textbf{evaluation protocols}, and discuss \textbf{robustness} issues that deserve attention.
Specifically, we attempt to explore:
1) how many real-world scenarios are covered by existing datasets, 
2) how fair and comprehensive are the evaluation protocols,
and 3) how robust the advanced KBQA method is in real-world scenarios.
First, the KBQA dataset uses only a single KB as the answer source to collect questions.
Due to the fact-based storage, incompleteness, timeliness of the KB, it only supports a limited number of question types.
In addition, some complex queries that are close to human demands are hard to collect due to the limitations of commonly used collection methods.
We also discuss unrealistic assumptions in some datasets, which compromises the comprehensiveness and effectiveness of the dataset.
% Besides, the issue of quality assurance of the dataset cannot be ignored for the correctness of model training and evaluation.

Second, several aspects of the KBQA evaluation protocols still fall short of reality.
We reflect on the shortcomings of evaluation metrics, discuss whether the evaluation is fair enough and how robustness is evaluated.
Because the characteristics of KBQA dataset construction limit the amount and distribution of training data, robustness for real-world scenarios is a challenge that needs to be carefully evaluated.
We summarize robustness challenges, such as schema-level generalization, paraphrase adaptation, and cross-dataset transfer, but existing evaluation protocols and solutions are inadequate for them.
% , where Hits@1 is not applicable to questions with multiple answers, and time evaluation is less discussed.

% Therefore, generalization to unseen scenarios and adaption to linguistic variation become key real-world challenges.
Third, to compensate for the lack of evaluation and solutions on robustness issues, we conduct experiments and analyses, where we propose a data augmentation method named \textbf{GAIN}, which improves 2.7 and 16.9 points in F1 compared to previous model on GrailQA and GraphQuestions with schema-level generalization, respectively.
It also improves 12.0 points in Hits@1 for relation linking task on SimpleQuestions-Balance with generalization.
Meanwhile, it has the potential to bring better capabilities of paraphrase adaptation to the KBQA model.
These results suggest that the data augmentation of GAIN is an effective way to improve the robustness.
Nevertheless, better evaluation and solutions for robustness are still open issues and deserve further exploration.
In particular, the difficult cross-dataset transfer means that dataset construction needs further reflection.
% Meanwhile, the ability of advanced KBQA models to reach dataset transfer paraphrase adaptation is still worth exploring.

==> backup/introduction0118.tex <==
Knowledge base question answering (KBQA) aims to answer natural language questions based on knowledge bases (KBs) such as DBpedia \cite{Lehmann15dbpedia}, Freebase \cite{bollacker08freebase} and Wikidata \cite{vrandecic14wikidata}. 
It allows users to query the KB through natural language without having to learn a complex formal query language.
Extensive research has been conducted on KBQA benchmarks and models \cite{lan21complex}.
% , with datasets ranging from small, single-hop to large, multi-hop with numerical operations.
% While the benchmarks continue to grow in size and query complexity, 
While KBQA models continue to achieve higher scores on benchmarks, the significance of the model progress only holds if the benchmark is close to real-world use. 
However, there has been far less discussion of benchmark than model, leaving less progress in data collection methods and evaluation protocols.
% However, benchmarks' data collection methods and evaluation protocols are virtually unchanged.
Most importantly, the lack of reflection on the whole benchmark building process leaves many real-world situations under-appreciated.
Their rigid query patterns and abbreviated evaluation are hard to satisfy diverse QA requirements in reality.
% KBQA benchmarks usually involve only rigid query patterns and abbreviated evaluation metrics, but the QA requirements in reality are diverse and difficult to summarize.
% In this work, we argue that KBQA benchmarks do not yet simulate real-world scenarios well.
Thus, unlike previous model-centric survey papers \cite{lan21complex,gu2022knowledge}, we systematically investigate the practicality of KBQA benchmarks by examining the \textbf{dataset construction} and \textbf{evaluation protocols}, and also explore the rarely considered \textbf{robustness} issues.
Specifically, we attempt to explore:
1) what scenarios in reality are covered or ignored by existing datasets, 
2) how fair and comprehensive are current evaluation protocols,
and 3) how robust the advanced KBQA models are in real-world scenarios.

% First, KBQA datasets rely on a single KB as the only source of answers, resulting in a limited number of questions and the exclusion of other types of questions.
% However, due to the fact-based storage, incompleteness, timeliness of the KB, it only supports a limited number of question types.
% In addition, the commonly used collection methods based on graph search do not cover the complex queries in QA requirements.
% First, the construction of KBQA datasets relies on individual KBs and question collection methods.
First, KBQA dataset construction depends on the capacity of the KB and the data collection method.
However, the fact-based storage, incompleteness, and timeliness of individual KB decides the available knowledge is limited.
Meanwhile, the properties of common question collection methods limit the complexity and quantity of the collected questions.
Both the KB and the collection make it difficult to outline user requirements in existing datasets.
% We also discuss unrealistic assumptions in some datasets, which compromises the practicality of the dataset.

Second, KBQA evaluation protocols are not fair and comprehensive enough.
It is reflected in unreasonable performance metrics, missing efficiency metrics, unfair model comparisons with different settings, and inadequate evaluation of robustness.
Especially for limited training data, robustness is a practical challenge that needs to be carefully evaluated.
We summarize robustness challenges, including a) generalization for unseen domains at the schema level, b) paraphrase adaptation for diverse linguistic variations, and c) the most demanding cross-dataset transfer with unseen schema, query patterns and linguistic styles.
Yet, both evaluation protocols and solutions are inadequate for them.

Finally, to compensate for the lack of evaluation on robustness issues, we conduct experiments and analyses, where we propose a data augmentation approach named \textbf{G}raph se\textbf{A}rch and quest\textbf{I}on generatio\textbf{N} (\textbf{GAIN}).
For schema-level generalization, it improves 2.7 and 16.9 points in F1 compared to previous state-of-the-art on GrailQA and GraphQuestions respectively, and also improves 12.0 points in Hits@1 for relation linking task on SimpleQuestions-Balance.
Meanwhile, it has the potential to bring better adaptability of paraphrase to KBQA models with a relative decrease of 7.6\% in the standard deviation of F1 scores of paraphrases on GrailQA.
It also drives performance advances for cross-dataset transfer.
However, robustness challenges are far from solved.
In particular, we show multiple large-scale pre-trained models, including GAIN, are still difficult to transfer to the unseen human-curated scenario without annotation data.
It calls for benchmark to collect more representative training data and to present more realistic challenges in the evaluation protocol.

% It demonstrates the inadequacy of existing datasets in reflecting diverse user requirements.

% In particular, we show that multiple large-scale pre-trained methods, including GAIN, are still difficult to transfer to the unseen human-curated dataset WebQSP without fine-tuning.
% It reveals the limitations of existing large-scale benchmarks and the significant differences between datasets.



% These experiments, trained and evaluated on existing benchmarks, show that GAIN achieves state-of-the-art performance.


% a strong and generalizable KBQA approach.
% These results also suggest that the data augmentation of \textbf{GAIN} is an advanced approach for existing benchmarks.


% However, this promising progress is fragile outside the scope of existing evaluation protocols and obscures deeper robustness challenges.
% We show that GAIN pre-trained on large-scale datasets is difficult 
% to transfer to an unseen human-curated scenario, and this challenge is related to the significant differences between the datasets.
% It reminds us to further think about whether KBQA benchmarks reflect diverse user requirements.


% We argue the drop represents significant differences between data collection methods.
% that it reveals significant differences among KBQA datasets and 
% Nevertheless, better evaluation and solutions for robustness are still open issues and deserve further exploration.
% In particular, we find that large-scale pre-trained models are difficult to transfer to new scenarios, revealing significant differences between KBQA datasets and reminding us to further reflect on the dataset construction process.

